Generative Parameter Sampler For Scalable Uncertainty Quantification

Uncertainty quantification has been a core of the statistical machine learning, but its computational bottleneck has been a serious challenge for both Bayesians and frequentists. We propose a model-based framework in quantifying uncertainty, called predictive-matching Generative Parameter Sampler (GPS). This procedure considers an Uncertainty Quantification (UQ) distribution on the targeted parameter, which matches the corresponding predictive distribution to the observed data. This framework adopts a hierarchical modeling perspective such that each observation is modeled by an individual parameter. This individual parameterization permits the resulting inference to be computationally scalable and robust to outliers. Our approach is illustrated for linear models, Poisson processes, and deep neural networks for classification. The results show that the GPS is successful in providing uncertainty quantification as well as additional flexibility beyond what is allowed by classical statistical procedures under the postulated statistical models.

==> abstract.tex <==
% !TEX root=./neurips_2019.tex
\begin{abstract}
Uncertainty quantification has been a core of the statistical machine learning, but its computational bottleneck has been a serious challenge  for both Bayesians and frequentists. We propose a model-based framework in quantifying uncertainty, called \emph{predictive-matching Generative Parameter Sampler} (GPS). This procedure considers an \emph{Uncertainty Quantification} (UQ) distribution on the targeted parameter, 
which is defined as the  minimizer of a distance between the empirical distribution and the resulting predictive distribution. This framework adopts a hierarchical modeling perspective such that each observation is modeled by an individual parameter. This individual parameterization permits the resulting inference to be computationally scalable and robust to outliers. Our approach is illustrated for linear models, Poisson processes, and deep neural networks for classification. The results show that the GPS is successful in providing uncertainty quantification as well as additional flexibility beyond what is allowed by classical statistical procedures under the postulated statistical models.
%model based framework within uncertainty  quantified with remarkable statistical formalism.




%The results show that the performance of the GPS is  competitive compared to well-known baseline models. 

%In particular for the MNIST data set, the classification error rate can be reduced to $0.12\%$ (lower than the state-of-art result, $0.21\%$) after accounting for the UQ. 

%generator function of the parameter in a given model, and this generator transforms a random variable 
%As an vignette, we consider the Maximum Mean Discrepancy Measure (MMD) as a special case in our framework. 


%can be applied to measure the difference between a sample and a hypothesized distribution or the difference between two or more samples in arbitrary, not necessarily equal dimensions.

%Experiments validate the potential of the framework through qualitative and quantitative evaluation of the generated samples.
\end{abstract}

==> background.tex <==
\section{Background}




==> conclusions.tex <==
% !TEX root=./neurips_2019.tex
\section{Conclusions}


==> experiments-mnist.tex <==
% !TEX root=./neurips_2019.tex

{\color{red} Draw figures... To explain the structure for the CNN.}  

\paragraph{Uncertain images.} We first describe what we mean by \emph{uncertain} images. Very intuitively, uncertain images are images where the classification probabilities are `fluctuating', in the sense that the values can appear from anywhere between $0$ and $1$. This can be seen from Figure \ref{fig:wrong}. Contrast this to 'certain images' where the classification probabilities do not `fluctuate' widely, (confer Figure \ref{fig:correct}. In order to carry out our experiment, we define formally those images that are uncertain in the following manner. We propose a \emph{Uncertainty Quantification Criterion} (UQC) for each class $h$ and an image $X$, denoted by $t_h$,  that is given as
\begin{eqnarray}\label{eq:t_h}
    \mathbb{P}_z\left[ C_h(X,z)< t_h \right] = 5\%,
\end{eqnarray}
where $C_h(X,z)$ is the classification probability of the class $h$, i.e., $C_h(X,{\bf z})= \exp\{G_h(X,{\bf z})\}/\sum_{l=1}^H \exp\{G_l(X,{\bf z})\}$ for $h=1,\dots,H$. Now we call an image ``Uncertain'' if  every $t_h$ corresponding to the image does not exceed 50\%. If an image is not ``Uncertain'', we call it ``Certain''. 


In Table \ref{tab:results}, we report the prediction performance of the standard procedure and our GPS procedrue. We see that the GPS procedure (0.72\% and 0.69\%) achieves competitive classification performance compared with the standard CNN procedures (0.79\%). The classificaiton tasks for the GPS are implemented by using the mean of the classification probabilities based on the UQ distribution, i.e., $\mathbb{E}_{\bf z}\left [ C_h(X,{\bf z}) \right]$ for $h=1,\dots,H$.


We use an extended CNN as generator, and it is trained using the training dataset. Prediction is carried out on a test dataset that excludes the uncertain test images. We see from Table xxx that the classification performance is significantly improved ($0.72\%$ to $0.122\%$ and $0.69\%$ to $0.154\%$). The third column shows that the proportion of the uncertain images is indeed low, just approximately $2\%$ to $3\%$. This means that by discarding a small proportion of  (uncertain) images, our performance of the classification can be dramatically improved.      

Once we have identified the uncertain images, we discard them.
Overconfident predictions on unseen classes in classifications are problematic and calls for caution. In an ideal situation, we would like the GPS to detect higher uncertainty when the test data significantly differs from the training data. To check if the GPS inherits this desirable property, we remove images of digits ``1'' in training steps for neural network classifiers. Then, we compute the  uncertainty in classification probabilities evaluated from unused images, which is digit ``1''. We observe that these values fluctuate with high uncertainty. This can be seen in Figure \ref{fig:without1}.
%\paragraph{Description of data.}
\subsection{MNIST}
We evaluate the performance of the GPS methodology on classification tasks using MNIST [XX] and CiFAR [XX] data sets. Our goal is to illustrate the applicability of quantifying uncertainty in these basic tasks. 

\begin{table}[htbp]
\caption{Test error rates under uncertainty quantification. \label{tab:results}
}
\centering
\begin{tabular}{l|ccc} 
\hline
\multicolumn{4}{c}{{\bf MNIST} } \\
\hline
Method & Error Rate (Full)& Error Rate (w\slash o ``Uncertain'' )& \% of ``Uncertain''\\
\hline
Standard CNN & 0.79\% &  &      \\
CNN-MCDrop & 0.80\% & 0.30\% & 2.05\% \\
CNN-GPS ($r=0.5$) & 0.72\% & 0.12\% & 2.99\%     \\
CNN-GPS ($r=0.25$) & 0.69\% & 0.15\% & 2.27\%   \\
%CNN-GPS ($r=0.125$) & 0.79\% & 0.132\% & 2.08\%   \\
%CNN-GPS (C, r=0.5) & \% & \% & \%     \\
%CNN-GPS (C, r=0.25) & \% & \% & \%   \\
\hline
\hline
\multicolumn{4}{c}{{\bf CiFAR10} } \\
\hline 
Standard ResNet & 16.50\% & &  \\
ResNet-MCDrop & 16.65\% & 10.37\% & 13.83\% \\
ResNet-GPS ($r=0.5$) & 15.95\% & 6.811\% & 22.48\% \\
ResNet-GPS ($r=0.25$) & 17.36\% & 7.892\% & 24.54\% \\

\hline 
\end{tabular}
\end{table}


\begin{table}[htbp]
\caption{ Training without one class }\label{tab:uncertain}
\centering
\begin{tabular}{l|cc} 
\hline
\multicolumn{3}{c}{{\bf MNIST} } \\
\hline
Method & \% of ``Uncertain'' from digit ``1'' & \% of ``Uncertain'' from random noise \\
\hline
CNN-MCDrop & 68.90\% & 69.76\% \\
CNN-GPS  & 97.27\%  & 97.28\% \\
\hline
\hline
\multicolumn{3}{c}{{\bf CiFAR10} } \\
\hline
ResNet-MCDrop & 53.50\% & 47.53\%  \\
ResNet-GPS  & 72.30\% & 77.24\% \\
\hline

\hline
\end{tabular}
\end{table}



%\begin{figure}
%    \centering
%        \includegraphics[width=5in, height = 1.2in]{independent_without_outliers3.pdf}
%       \caption{An example with independent covariates. {\color{red} Move this to the appendix.} } \label{fig:independent}
%\end{figure}       





\begin{figure}
    \centering
        %\includegraphics[width=2.4in, height = 1in]{correct4}
        %\includegraphics[width=2.4in, height = 1in]{correct7}
        \includegraphics[width=2.4in, height = 1in]{correct1}
        \includegraphics[width=2.4in, height = 1in]{correct9}
       \caption{Two examples of MNIST data set for ``Certain'' cases. The yellow-colored numbers  on the left-side of the digit images indicate the the true labels and the green-colored probability indicate the mean of classification probability  of the true class. The boxplots illustrate the UQ distributions of the classification probabilities and the red crosses in the boxplot show  the sampled classification probabilities from the UQ distribution.} \label{fig:correct}
\end{figure}       

\begin{figure}
    \centering
        %\includegraphics[width=2.4in, height = 1in]{wrong_uncertain9}
        %\includegraphics[width=2.4in, height = 1in]{wrong_uncertain8}
        \includegraphics[width=2.4in, height = 1in]{wrong_uncertain7}
        \includegraphics[width=2.4in, height = 1in]{wrong_uncertain5}
       \caption{Two examples of MNIST data set for ``Uncertain'' cases. The description is the same with that in Figure \ref{fig:correct}.} \label{fig:wrong}
\end{figure}       


\begin{figure}
    \centering
        \includegraphics[width=2.4in, height = 1in]{digit1_10}
        \includegraphics[width=2.4in, height = 1in]{digit1_6}
       \caption{Two examples of classification results with uncertainty qunatification where the images of the digit ``1'' are unused in the training step. For each class $h$, the value of $t_h$ in \eqref{eq:t_h}  is marked by the blue ``\texttt{x}'' on the boxplots.} \label{fig:without1}
\end{figure}       


==> experiments-spatial.tex <==
% !TEX root=./neurips_2019.tex
%\subsection{Spatial}
%\paragraph{A simple motivating example.} 
%Suppose we are interested to formulate a classical Poisson regression which dictates
%\begin{align}
%y_i\mid\lambda_i \sim \mathrm{Poisson}(\lambda_i).
%	\end{align}
%within a GPS framework. Let $\lambda_i=\exp(a_i+b_i\cdot\textbf{x}_i)$. Now we set
%\begin{align}
%\mathbb{R}^2\ni\theta_i = \begin{pmatrix} a_i \\ b_i \end{pmatrix}= \begin{pmatrix} \phi_1 Z_i + \phi_2 Z_2^2 \\ \phi_3 Z_i^3 + \phi_4 Z_i^4 \end{pmatrix}
%\end{align}
%We note that in this motivating example, $(\phi_1,\phi_2,\phi_3,\phi_4)$ are the `shared parameters' for across the samples $y_1,y_2,\hdots,y_n$.

==> experiments-synthetic.tex <==
% !TEX root=./neurips_2019.tex
\section{Experiments on MNIST and CiFAR10 Data Sets}
%\subsection{Illustration with Synthetic Data}




==> introduction.tex <==
% !TEX root=neurips_2019.tex
\section{Introduction}
\label{introduction}
\paragraph{Purpose of the present paper.} %The purpose of this paper is 
We propose a general framework to quantify uncertainty on the inference of parameters. This is conducted by searching an Uncertainty Quantification (UQ)  distribution, of parameters in interest, that minimizes a \emph{ distance} between the predictive distribution based on the UQ distribution and the empirical distribution.  Since directly evaluating the UQ distribution function (or density function) is computationally challenging, we consider a parameter generator that generates parameter samples that follow the minimizer UQ distribution to ease the computational difficulty. In this sense, we call the proposed procedure (predictive-matching) \emph{Generative Parameter Sampler} (GPS).

%but abstracts the notion of a different \emph{distance} that measures the predictive distribution and its empirical counterpart. Specifically, our proposed approach can be seen as non-parametric type of Type II that minimizes a reasonable and efficient approximation of the MMD distance. 


%In this paper, we propose a framework to draw inferences that follows this theme, but abstracts the notion of a different \emph{distance} that measure the predictive distribution and its empirical counterpart. 


The proposed GPS can be considered as a generalized nonparametric version of \emph{type II maximum likelihood} (henceforth known as type II in this paper) \citep{Berger:1985}. In Type II maximum likelihood, parameter (or hyperparameter) estimation is carried out by minimizing the \emph{Kullback-Leibler} (KL)-divergence between the empirical density and the predictive density marginalized out by a parametric distribution of the parameter. In contrast, the GPS has no parametric assumption on  the parameter distribution in evaluating the predictive distribution, and the discrepancy measure for the GPS is not necessarily KL-divergence. Unlike the standard type II MLE, the procedure of the GPS evaluate a generator function that transforms 

%In this paper, we propose a framework to draw inferences that follows this theme, but abstracts the notion of a different \emph{distance} that measure the predictive distribution and its empirical counterpart. Our proposed approach can be seen as a generalization of Type II maximum likelihood which uses the Kullback-Leibler as a distance measure. 


This new resulting framework is applicable for large scale uncertainty quantification (e.g., generalizing confidence interval and prediction interval embracing uncertainty) for complex models (e.g., deep learning classification models). In detail, our contributions are as follows:
\begin{itemize}
    \item (New framework) We propose a framework for drawing inferences through the minimization of MMD distance within the Type II methodology in place of the Kullback–Leibler divergence in the classical setup. We posit that the true parameter is drawn from a generating process, which we call the \emph{generator} (confer definition \ref{eq:predictive-distribution-Q_G}).
    \item (High quality UQ) We show that our framework in generating parameters yields high quality \emph{model-based} predictive uncertainty estimates. We take the view that a model-based approach is crucial to describe, predict, and facilitate interpretability of the generated samples. This differs from standard methods used to generate pseudo samples, e.g., the {W}asserstein Generative Adversarial Networks \citep{WGAN:2017} whose procedures do not emphasize on a set of modeling assumptions regarding the generation of observations. 
    \item (Independence structure and its implications) By construction, GPS induces a set of \emph{fully} independence structure (Figure \ref{fig:gps-vs-standard}\,(a)) in contrast to standard Bayesian models (Figure \ref{fig:gps-vs-standard}\,(b)). This artefact (Figure \ref{fig:gps-vs-standard}\,(a)) makes it scale since it allows training of the generator using subsamples via standard optimization algorithms. We demonstrate that due to this individualized framework of generating parameters, GPS is capable of giving estimates when the model is misspecified (Section xxx).
	\item (Ease of implementation) We show that training GPS does not require a complicated design of the network architecture (see Algorithms xxx, yyy). One appealing aspect of GPS is that it \emph{bypasses} the application on invertibility and tractable Jacobians of the transformation \citep{Rezende:2015,Berg:2018}. This is because GPS directly measures the \emph{probability distance} between observe samples and generated samples in contrast to the \emph{density} functions between them.
\end{itemize}



==> proposedmethod.tex <==
% !TEX root=./neurips_2019.tex
\section{Generative Parameter Sampler}
\label{sec:gps}
\paragraph{Quick recap.} The main idea of GPS is to draw inferences that follows this idea of Type II, but abstracts the notion of an MMD distance that measures the predictive distribution and its empirical counterpart. At the high level, our proposed approach can be seen as non-parametric type of Type II that minimizes a reasonable and efficient approximation of the MMD distance. 

\paragraph{GPS - Generating parameters and not samples.} We first posit that our observations $y_i\mid\theta_i$ comes from a distribution $f_{\theta_i}$. We define a random variable $Z$, which with a tractable density function (such as $Z\sim N(0,I)$), and pass it through a parametric function $G$, where we take it to be a neural network of some kind. The function $G:\mathbb{R}^{q}\rightarrow\mathbb{R}^{p}$ and call $G$ the \emph{generator}. For $i=1,\dots,n$, we further let $\theta_i:=G(Z_i)$ and denote $\pi_G$ as the probability density function corresponding of $\theta_i$. The predictive distribution for GPS can thus be written succinctly as
\begin{align}
\widetilde f_{G,i}:=\int f_{\theta_i}(y_i)\pi_G (d\theta_i)
\end{align}
where $y_i$ is the $i$-th observation. We then generate the parameters $\theta_i$ following a certain distribution $\pi_G$. 


\begin{definition}
The optimal parameter of GPS is defined as the minimizer $G^*$ of a distance between the predictive distribution $\widetilde f_G$ and the empirical distribution $f_n$:
\begin{eqnarray}\label{eq:GPS}
\widehat \phi = \argmin_\phi \emph{\textrm{MMD}}(f_n, \widetilde f_{G_\phi})
\end{eqnarray}
where the generator $G_{\phi}$ is a neural network model with parameter $\phi$.
\end{definition}

\paragraph{Explaining Type II.} The methodology of drawing inferences within the Type II maximum likelihood framework (henceforth abbreviated as Type II) has been treated at various levels of model complexitiy by a number of authors (confer \cite{Berger:1985}). If the empirical distribution admits a distribution $f_n$, say, then parameter estimation from Type II can be recast as minimization of the Kullback-Leibler divergence between $f_n$ and a predictive distribution $\widetilde f$. The predictive distribution $\widetilde f$ is obtained by via the marginal likelihood function, obtained by first integrating over the latent parameters $\theta$.


This setting has been commonly considered in classical statistics and machine learning applications. By imposing a prior on $\theta$, Bayesian linear regression models utilize posterior inference via the conditional distribution of $\theta$, and the conditional uncertainty on the parameter space, given the data, is identified through the posterior distribution. 

In contrast, as illustrated in Figure XXX  the GPS follows an individualized parameterization assuming that there exists a true parameter generating law $\pi^*$ for each $\theta_i$ for $i=1\dots,n$. This setup can be considered as a slight generalization of classical  frameworks in a sense that a points mass $\pi^*$ at a fixed $\theta_0$ results in a frequentist's model that assumes the existence of the true parameter $\theta_0$ that is fixed and unknown. Under this individualized parameterization, the GPS procedure estimates the parameter generating process $\pi^*$ by minimizing a distance between the predictive distribution and the observations. The main reason of deploying the individualized parameterization is that a sclable algorithm can be used under the \emph {fully} independent structure between the observation. This means that a small set of generated fake samples of $y$ can be used to approximate the MMD in optimization. In contrast, under the classical setup as in Figure XXX, the computation of a distance in GPS requires a generation of  a full set ($n$-sized) of fake samples to completely quantify the conditional reasoning $\theta\vert y_1,\dots, y_n$, which is computationally demanding for large-sized data sets.     

In classical models in statistics and machine learning, the individualized parameterization has not been commonly used in practice due to some reasons. In Bayesian statistics, Dirichelet Process Mixture (DPM) models follow the individualized parameterization by imposing a DPM prior on the parameters, but the MCMC computation of the posterior distribution is extremely demanding especially in large-sized data set; every iteration the MCMC algorithm samples $n$ number of $\theta$s. Also, the DPM models have a nature of discreteness in posterior distribution, so it can be used to solve clustering problems without specifying the number of clusters. However, the discreteness of the posterior distribution based on DPMs hurdles the practical use of DPM to more general settings where the posterior space is continuous. For these reasons, we do not examine the DPM models further in sequel.

In frequenstist's frameworks, the individualized parameterization is also not considered because it is assumed that the true parameter is fixed without any stochastic properties on the parameter. While some hierarchical models like random effect models are considered in practice, the main focus of frequentist's hierarchical models is not in estimating the distribution of $\theta$, but in reducing some random effects that may affect the estimation of parameters in interest.    

The Gaussian mean model, $y_i=\theta_i+\epsilon_i$, also assumes the individualized parmeterization. However, this model is not  designed to analyze real data sets, but its usage is only restricted in investigating theoretical properties of various statistical procedures. These include risk minimization (XXX) , high-dimensional variable selection (XXX) and nonparametric function estimation (XXX). For this reason, we do not consider the Gaussian mean model further in this article.      



\subsection{Objective function}
Using the definition of MMD \citep{gretton2012kernel}, it can be shown that 
\begin{eqnarray}
\label{eq:MMD}
\mbox{MMD}(f_n, \widetilde f_G) = -\frac{2}{n}\sum_{i=1}^n\mathbb{E}_{\widetilde Y_i\sim \widetilde f_{G,i}}\left[k(y_i,  \widetilde Y_{i} )  \right] + \frac{1}{n}\sum_{i=1}^n\mathbb{E}_{\widetilde{Y}_i,\widetilde{Y}_i'\overset{i.i.d.}{\sim}\widetilde f_{G,i}}\left[k (\widetilde Y_{i}  , \widetilde Y^{\prime}_{i} )  \right],
\end{eqnarray}
where $k(\cdot,\cdot)$ is a positive-definite kernel. In this article, we use a Gaussian kernel $k(x_1,x_2) = \exp\{-\Vert x_1 - x_2\Vert^2_2\}$ as canonical choice. %The original MMD is supposed to be maximized, so it should contain minus sign in \eqref{eq:MMD}, but to use the MMD as a distance, we ignore the minus sign.



\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.6\linewidth]{gps-graphical-model.pdf}
  \caption{Individualized parameterization}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.53\textwidth}
  \centering
  \includegraphics[width=.6\linewidth]{classic-graphical-model.pdf}
  \caption{Globalized parameterization (Bayesian and frequentist)}
  \label{fig:sub2}
\end{subfigure}
\caption{\emph{Scalability of GPS.} Our method of generating samples from the generator $G$ induces a set of fully independent structure amongst the observations $\{{y_i}\}_{i=1}^n$. This is in contrast to the standard model setting $\textrm{(b)}$, where observations are conditionally independent given the parameters. In the generative paradigm of $\textrm{(b)}$, $\theta$ is first sampled which is then followed by generating $n$ samples. This procedure incurs huge computational burden when $n$ is large and is ubiquitous in some well known Bayesian analysis, such as the approximate Bayesian computation (ABC) \citep{Tavare:1997,Sunnaker:2013,Espen:2019}. Our proposed GPS model is scalable and flexible as it inherits the independence structure $\textrm{(a)}$ since for each $\theta_i$, one can sample $y_i$ independently. Hence, no sampling is needed for the full set of observations as in $\textrm{(b)}$ for each $\theta_i$.}
\label{fig:gps-vs-standard}
\end{figure}


\subsection{Learning}
\begin{algorithm}
\caption{GPS Algorithm.}\label{alg:alg}
\begin{algorithmic}
\State Set the learning rate $\gamma$, $n_0$, $M$, $J$, and set $t=1$
\While{the stop condition is not satisfied} 
\State{Set $J_{\phi^{(t)}}=0$.}
\State{Sub-sample $n_0$ samples from the original data set.}
\For{$m = 1,\dots,M$}
\State{Independently generate $z_i^{(m)}$ from $N(0,I_q)$.}
\State{Set $\theta_i^{(m,t)}=G_{\phi^{(t)}}(z_i^{(m)})$.}
\For{$j=1,\dots,J$}
\State{Independently generate $\widetilde y_{ G_{\phi^{(t)}} ,i(j) }^{(m)}$ from $f_{ \theta_i^{(m,t)} }$ for $i=1,\cdots,n_0$.}
\State{Set $J_{G_{\phi^{(t)}}} = J_{G_{\phi^{(t)}}} + \frac{\partial}{\partial\phi}\widehat{d}(f_{n_0},\widetilde f_{G_{\phi}})\big\vert_{\phi = \phi^{(t)}}$, where $\widehat d$ is a Monte Carlo approximation of MMD.  }
\EndFor
\EndFor
\State{$\phi^{(t+1)} = \phi^{(t)} - \gamma J_{\phi^{(t)}}$.} 
\State{Set $t = t+1$.}
\EndWhile
\end{algorithmic}
\end{algorithm}

\section{Applications}
%Different specifications of $G$ leads to major areas of applications.
       
\subsection{Linear regression}
Consider a linear regression model that contains a univariate response variable $y_i$ and $p$-dimensional predictor $X_i$ for $i=1\dots,n$, and its regression coefficients is denoted by $\theta\in\mathbb{R}^p$.   
\begin{eqnarray*}
 y_i = X_i^T\theta + \epsilon_i,
\end{eqnarray*}
where $\epsilon_i\sim N(0,\sigma^2)$. In the framework of the GPS, we consider an individualized parameterization such that the uncertainty on  $\{\theta_i,\sigma^2_i\}_{i=1,\dots,n}$ is quantified by an UQ distribution $\pi^*$. This UQ distribution is constructed in a generative sense, and the generator $G(Z_i)=\{\theta_i,\sigma^2_i\}$, such that $G:\mathbb{R}^q\to \mathbb{R}^p\times\mathbb{R}$, generates the parameters without identifying the density function $\pi^*$ itself.

\begin{figure}
    \centering
        \includegraphics[width=0.9\textwidth]{scissor_post.pdf}
       \caption{The scatter plot of a scissors example (left); Bayesian posterior distribution of $\theta$ (middle); the UQ distribution from the GPS (right).} \label{fig:standard}
\end{figure}

To examine the different properties of the GPS from the standard framework, we consider an one-dimensional simple linear regression example ($p=1$), where $X_i$ is generated from i.i.d. standard Gaussian and the true data-generating process follows $y_i=\gamma_iX_i - (1-\gamma_i)X_i  +\epsilon_i$, where $\gamma_i\sim Bernoulli(1/2)$ and $\epsilon_i\sim N(0,0.2^2)$ for $i=1,\dots,n$. The resulting scatter plot of a synthetic data set is illustrated in the first column of Figure \ref{fig:standard}. In  this example, the classical globalized parameterization is not capable of capturing the scissors-look like shape. As a consequence, as depicted in the second column of Figure \ref{fig:standard}, the standard posterior distribution of $\theta$ from a uniform prior is  concentrated on zero, and this posterior behavior is ill-positioned against the true nature. In contrast, the third column of Figure \ref{fig:standard} shows that the UQ distribution derived from the GPS exactly captures the bimodal shape of the true distribution on the slope parameter ($\theta_1=1$ with $50\%$ and $-1$ with $50\%$). This example shows that compared to standard procedures, the GPS covers a wider range of true data-generating process within a family of models (linear regression models in this case).
%\begin{figure}
%    \centering
%        \includegraphics[width=0.65\textwidth]{scis%sors_fit.pdf}
%       \caption{} \label{fig:standard}
%\end{figure}       


To examine how robust the GPS is to the influence of outliers, we consider an example as follows: the predictor $X_i\in\mathbb{R}^{p}$ with $p=20$ is generated from i.i.d $N(0,\Sigma)$, where $\Sigma_{jk} = 0.5$, if $j\neq k$ and $\Sigma_{jj} =1$ for $j,k=1,\dots,20$, $\epsilon_i\sim N(0,1)$, and $n=200$. We compare the UQ distribution of the GPS with the Bayesian posterior distribution with a uniform prior and its approximated variational posterior distribution ({\color{red}cite}). The variational posterior distribution of each parameter is modeled by independent Gaussian distribution, and we use \texttt{varbvs} \texttt{R} package to implement  the variational inference. The 5\% of response samples are randomly set to be outliers and they are contaminated with additive extra noises generated from Cauchy distribution with scale $3$, and the results are illustrated in the top row of Figure \ref{fig:outliers}. While the existence of outliers significantly distorts the posterior behavior due to its dependence structure that connects all observations to a single parameter $\theta$, in the GPS the observed outliers only affect their corresponding parameters in the individualized parameterization. This property results in more robust inference to outliers, and the UQ distribution of the GPS attains a stable contraction on the true regression coefficients under the existence of outliers. In contrast, the Bayesian posterior and its variational approximated distributions are highly unstable and departed from the truth.   

\begin{figure}
    \centering
        %\includegraphics[width=0.9\textwidth]{outliers3.pdf}
        \includegraphics[width=5in, height = 1.2in]{outliers3.pdf}
        \includegraphics[width=5in, height = 1.2in]{without_outliers3.pdf}
       \caption{An example under the existence of outliers (top) and  under the absence of  outliers (bottom) for the UQ distribution of the GPS (left), the Bayesian posterior distribution (middel), and the approximated posterior distribution by the variational inference (right). The true coefficient values are marked by red ``\texttt{x}''. } \label{fig:outliers}
\end{figure}       

We also consider a classical scenario where the  assumptions for the Bayesian linear model are satisfied well. We examine the same setting used in the previous outlier example, but this classical example contains no outliers. The results in the bottom row of Figure \ref{fig:outliers} show that the UQ distribution of the GPS behaves similarly with the Bayesian posterior distribution. On the other hand, the variational posterior distribution underestimates the target distribution, and the mean of the approximated posterior is more biased towards zero. This is because the variational inference procedure ignores the correlation structure of the posterior space, so the mean field approximation does not approximate well the target posterior in this example. When the covariates are independent (so that the parameters in the resulting posterior space are also independent), the variational approximation is quite accurate, and the results from the independent predictors are reported in the Appendix. 


\subsection{Poisson processes with random intensities}
We show the applicability of GPS in the context of Poisson processes inheriting random intensities. These are when the outputs are counting numbers, i.e. non-negative integers, $y\in\mathbb{Z}_{+}$. 

For example, we may postulate that there are $L$ locations $\{{\ell}_i\}_{i=1}^L$ and the vectors $\{a_i\}_{i=1}^L$ of individual attributes (age, sex, income, etc.) as coordinates of the ``marked'' points $\{s_i\}_{i=1}^L$ in the product space $\mathcal{S}\equiv\mathcal{L}\times\mathcal{A}$ of ordered pairs $s = (\ell,a)$ of locations $\ell\in\mathcal{L}$ and attributed vectors, which are also called marks $a\in\mathcal{A}$. We model the $\{s_i\}_{i=1}^L$ as events of a Poisson random variable.

Formally, we consider an inhomogeneous Poisson process on a domain $\mathcal{S}$ which we take to be $\mathbb{R}^D$. The Poisson process is parameterized by an intensity function $\lambda(s):\mathcal{S}\rightarrow R^{+}$ where $\mathbb{R}^{++}$ indicates the positive real numbers. The random number of events in region $\mathcal{T}\subset\mathcal{S}$ is Poisson random variable with parameter $\lambda_{\mathcal{T}}=\int_{\mathcal{T}}\lambda(s)ds$. 

\begin{figure}
    \centering
        \includegraphics[width= 3.5in, height = 2.7in]{PoissonRegression0.pdf}
       \caption{ Poisson process example.  Generated samples by the GPS (black ``\texttt{x}'') and the observations (red ``\texttt{+}'') (upper left); the mean of the intensity evaluated by the GPS versus the truth (upper right); the true intensity on the spatial domain (lower left); the mean of intensity by the GPS on the spatial domain. } \label{fig:poisson}
\end{figure}       


In order to model the uncertainty of the intensity function $\lambda(x)$ via a kernel, the traditional approach is to use the Cox process \cite{kingman1993poisson}. A Cox process is defined via a stochastic intensity function $\lambda(x)$. The stochastic process to generate the intensity function is usually chosen to be a Gaussian process (GP) and some functionals thereof \citep{adams2009tractable,gunter2014efficient,lloyd2015variational,lloyd2016latent}.

To embed this in our framework, we let $\theta_i:=\lambda(s_i)$ and $\log \theta_i=G_\phi(s_i,Z_i)$, where $s_i\in\mathbb{R}^D$ for simplicity and set $Z_i\sim N(0,I_q)$, say. 



\subsection{Deep neural network for classification}
In image classification, Deep Neurual Network (DNN) models have been widely used by deploying convolutional layers [refXXXX], while the uncertainty quantification on the prediction of the classification still remains a challenging task. To solve this uncertainty quantification problem, we apply the GPS to the classification model with $H$ number of classes that follows: for $h=1,\dots,H$,
\begin{eqnarray}\label{eq:class}
\mathbb{P}[y_i=h] = \frac{\exp\{\theta_{hi}\}}{\sum_{u=1}^H\exp\{\theta_{ui}\}},
\end{eqnarray}
where $X_i\in\mathbb{R}^p$ is the the $i$-th predictor (or image) corresponding to $y_i$, and $\{\theta_{1i},\dots,\theta_{Hi}\}$ denotes the classifier of $X_i$ for each class. The classifier function  is commonly modeled by a DNN (e.g., CNN) by imposing $X_i$ as the input and $\{\theta_{1i},\dots,\theta_{Hi}\}$ as the output, and the cross entropy loss can be used to train the DNN in standard procedures. 

 For this application, we set the GPS as $\{\theta_{1i},\dots,\theta_{Hi}\} = G_\phi(\{X_i, Z_i\})$ such that $G_\phi: \mathbb{R}^{p+q}\to\mathbb{R}^H$, where  $\phi$ denotes the parameter of  the generator and $q$ is the dimension of $Z_i$ which follows $N(0, I_q)$. The only difference from this GPS setting and the standard DNN structures is that this generator embraces the randomness to the neural network by augmenting the random noise variable $Z_i$ into the input, so that the resulting NN is naturally random. After learning the parameters $\phi$ for the generator from the objective function in \eqref{eq:MMD}, the trained generator of the classifiers then generates the classification probabilities that captures the uncertainty in matching the predictions and the observations. 
 
 The figure shows a standard convolutional neural networks with input is an image and output is the class of the image (e.g. cat, dog, otter). There are 8 layers in the network: 1 input layer, 2 convolutional layers (Conv), 2 pooling layers (Pool), 2 fully connected layers (FC), and 1 output layer after softmax. A convolutional layer divides the current layer into sub-regions and connect neurons in the sub-region only to one neuron in the next layer.Pooling layer reduces the dimensions of the data by combining the outputs of neuron clusters at one layer into a single neuron in the next layer. Fully connect layer connect all neurons of the current layer to each neuron in the next layer. A softmax function is used to normalize the output, to map it to to probability value for class prediction purpose. Our proposed method is different in that it adds an randomness input $Z$ to last FC layer to make it as random variable, thus the network becomes a random function.
 
This GPS structure in Figure \ref{fig:cnn} achieves a computational advantage over the other uncertainty quantification procedures based on variational inference. These include inverse autoregressive flow (ref), NON-LINEAR INDEPENDENT COMPONENTS
ESTIMATION (ref) and normalizing flow (ref), and like the GPS these procedures also consider an idea of generator from a noise random variable. However, unlike the GPS, these procedures approximates the Bayesian posterior distribution of the DNN parameters that is usually extremely high-dimensional. For example, a simple one-layered feed forwarding neural network with $1,000$ nodes contains $(p+H)\times 1001$ number of parameters, and this number of parameters can be extremely large when $p$ is large or the number of nodes (and layers) is large. Constructing a neural network that transforms a random noise $Z\sim N(0,I_q)$ to such a high dimension (the number of parmeters in the target DNN) is a computationally challenging task. It may require more than billions of DNN parameters to train the generator when the target dimension is tens of thousands. In contrast, the GPS directly models the classifier function by using a DNN augmenting the random noise $Z_i$ into the input. Only difference from the deterministic DNN is that the input dimension is increased just by the dimension of $Z_i$,. This dimension can be controlled by the user, and in Section XX, we show that the performance of the generatoris not sensitive to the choice of the dimension of $Z$ in some examples.

%\section{Generative Neural Network Sampler}
%In a neural network setting, the number of parameters in a deep neural network is usually large. A direct application of GPS in Section \ref{sec:gps} to a deep neural network is practically challenging. The output dimension of the generator $G$ is the number of parameters in the deep neural network model, which is usually taken to be a large number. For example, if the input dimension is $p$ and the number of nodes is $1000$, and the output dimension is $d$, then the resulting number of parameters for the one-layered feed forwarding neural network is $(p+d)\times 1001$. This can be a very large number depending on the number of the layer or nodes and also when $p$ is large. Hence, we propose a special case of GPS to deal with this computational bottleneck which we term Generative Neural Network Sampler (GNS). 

%Instead of considering the weight and bias parameters in a neural network setting, we augment the input space with a set of random variables $(Z_1,Z_2,\hdots,Z_q)$ such that the output of the resulting neural network is random. For the case of convolutional neural network, our proposed framework is shown in Figure \ref{fig:gns}. Suppose the original input is denoted by $X\in\mathbb{R}^p$ and the resulting GNS can be defined as a neural network having $X$ and $Z$ as the input, i.e., $G(\{X,Z\}):\mathbb{R}^{p+q}\to\mathbb{R}^{d}$, 


\begin{figure}
\centering
  \includegraphics[width=2.7in, height = 1in]{cnn}
  \caption{The GPS for classification tasks using the CNN. }
  \label{fig:cnn}
\end{figure}%

%Neural network
%This section is an immediate consequence of our main model, GPS. In a nutshell, we place the generator $G$ on the network itself. 


% \subsection{A simple illustration}
% \begin{itemize}
% 	\item Poisson regression dictates
% 	\begin{align}
% 	y_i\mid\lambda_i \sim \mathrm{Poisson}(\lambda_i).
% 	\end{align}
% 	We further set $\lambda_i=\exp(a+b\cdot\textbf{x}_i)$.
% 	\item GPS $\theta_i = \lambda_i$\\
% 	\item Let $\lambda_i = G(Z)$
% \end{itemize}

	



==> relatedwork.tex <==
% !TEX root=./neurips_2019.tex
\section{Related work}

